$M^3EL$: A Multi-task Multi-topic Dataset for Multi-modal Entity Linking

Multi-modal Entity Linking (MEL) is a fundamental component for various downstream tasks. However, existing MEL datasets suffer from small scale, scarcity of topic types and limited coverage of tasks, making them incapable of effectively enhancing the entity linking capabilities of multi-modal models. To address these obstacles, we propose a dataset construction pipeline and publish $M^3EL$, a large-scale dataset for MEL. $M^3EL$ includes 79,625 instances, covering 9 diverse multi-modal tasks, and 5 different topics. In addition, to further improve the model's adaptability to multi-modal tasks, We propose a modality-augmented training strategy. Utilizing $M^3EL$ as a corpus, train the $\textit{CLIP}_{\textit{ND}}$ model based on $\textit{CLIP} (\textit{ViT}-\textit{B}-\textit{32})$, and conduct a comparative analysis with an existing multi-modal baselines. Experimental results show that the existing models perform far below expectations (ACC of 49.4%-75.8%), After analysis, it was obtained that small dataset sizes, insufficient modality task coverage, and limited topic diversity resulted in poor generalisation of multi-modal models. Our dataset effectively addresses these issues, and the $\textit{CLIP}_{\textit{ND}}$ model fine-tuned with $M^3EL$ shows a significant improvement in accuracy, with an average improvement of 9.3% to 25% across various tasks. Our dataset is available at https://anonymous.4open.science/r/M3EL.

==> raw_file/1-intro-raw.tex <==
\section{Introduction}
Multi-modal Entity Linking is a crucial research direction in Natural Language Processing (NLP) and Computer Vision (CV)~\cite{sevgili2022neural}. It aims to achieve cross-modal information integration and understanding by associating entities in different modalities (e.g., text, images, etc.), and to improve the accuracy of Information Retrieval~\cite{chang2006survey, martinez2020information} and Question-Answer systems~\cite{allam2012question, molla2006named}.

There are many limitations of current MEL datasets, which are summarised in Table~\ref{table:existing_datasets}. Firstly, existing datasets are generally small in scale; for instance, WIKIPerson~\cite{sun2022visual} involves 13K entities and WIKIDiverse~\cite{wang2022wikidiverse} covers 40K entities, which are insufficient for complex tasks. Secondly, the scope of modal tasks is restricted~\cite{hoffart-etal-2011-robust,moon-etal-2018-multimodal-named,gan2021multimodal}, primarily to $T_m-T_e$, $I_m-T_e$, or $I_m-(I+T)_e$, while neglecting other potentially valuable tasks such as $T_m-I_e$ and $T_m-(I+T)_e$. Additionally, most datasets are confined to single topics~\cite{guo2018robust,zhang2021attention}, such as person or news, and lack the ability to generalise across topics. These constraints significantly impede the development of MEL tasks.

\begin{table*}[!t]
\scriptsize
% \setlength\tabcolsep{0.5cm}
\centering
\begin{tabular}{c|l|cccc}
\toprule
\textbf{Task} &  \textbf{Dataset} & \textbf{Source} & \textbf{Topic} & \textbf{Size} & \textbf{Modality}  \\ \midrule

 & AIDA~\cite{hoffart-etal-2011-robust} & Wikipedia & Sports & 1K docs & $T_m\rightarrow T_e$ \\
 & MSNBC\cite{cucerzan-2007-large} & Wikipedia & News & 20 docs & $T_m\rightarrow T_e$ \\
 & AQUA\cite{milne2008learning} & Wikipedia & News & 50 docs & $T_m\rightarrow T_e$ \\
 & ACE2004\cite{ratinov-etal-2011-local} & Wikipedia & News & 57 docs & $T_m\rightarrow T_e$ \\
 & CWEB\cite{guo2018robust} & Wikipedia & Web & 320 docs & $T_m\rightarrow T_e$ \\
 & WIKI\cite{guo2018robust} & Wikipedia & Common & 320 docs & $T_m\rightarrow T_e$ \\
\multirow{-7}{*}{\textbf{EL}} & Zeshel\cite{logeswaran-etal-2019-zero} & Wikia & Common & - & $T_m\rightarrow T_e$ \\ \midrule
 & Snap\cite{moon-etal-2018-multimodal-named} & Freebase & Social Media & 12K captions & $T_m,I_m \rightarrow T_e$  \\
 & Twitter\cite{adjali-etal-2020-building} & Twitter users & Social Media & 4M tweets & $T_m,I_m\rightarrow T_e,I_e$ \\
 & Movie\cite{gan2021multimodal} & Wikipedia & Movie Reviews & 1K reviews & $T_m,I_m\rightarrow T_e,I_e$ \\
 & Weibo\cite{zhang2021attention} & Baidu Baike & Social Media & 25K posts & $T_m,I_m\rightarrow T_e,I_e$ \\ 
 & WikiDiverse\cite{wang2022wikidiverse} & Wikipedia & News & 8K captions & $T_m,I_m\rightarrow T_e,I_e$ \\ 
 & WikiPerson\cite{sun2022visual} & Wikipedia & Person & 50K images & $T_m,I_m\rightarrow T_e,I_e$ \\ \cmidrule{2-6}
\multirow{-7}{*}{\textbf{MEL}} & \textsc{$M^3EL$} & \makecell{Wikipedia, Wikidata, \\Dbpedia, Goodreads} & \makecell{Sports, Movies, Books, \\Person, Common} & 79K instances & $T_m,I_m,(I+T)_m\rightarrow T_e,I_e,(I+T)_e$ \\ \bottomrule
\end{tabular}
\caption{Overview of EL and MEL datasets. $T_m$ ($T_e$) and $I_m$ ($I_e$) represent the textual and visual contexts of mentions $m$ (or entities $e$) respectively, ``Manual'' denotes whether it is manually annotated, and ``Open'' denotes whether it is an open source.}
\label{table:existing_datasets}
\end{table*}

In this paper, we address these challenges by releasing the largest multi-task, multi-topic, multi-modal entity linking dataset, termed $M^3EL$. Specifically, the dataset contains 79,625 instances, significantly surpassing traditional datasets such as WIKIPerson~\cite{sun2022visual} and WIKIDiverse~\cite{wang2022wikidiverse}. Moreover, $M^3EL$ includes a comprehensive range of multi-modal tasks, including $T_m-T_e$, $T_m-I_e$, $T_m-(I+T)_e$, $I_m-T_e$, $I_m-I_e$, $I_m-(I+T)_e$, $(I+T)_m-T_e$, $(I+T)_m-I_e$, $(I+T)_m-(I+T)_e$. Finally, the dataset covers 5 topics: movies, common knowledge, person, books, and sports.

Baseline experiments indicate that existing models show limited performance on the $M^3EL$ dataset, with accuracy (ACC) ranging from 49.4\% to 75.8\%. The results suggest that despite the advances brought about by pre-trained language models, our dataset remains a challenging benchmark, underscoring the need for ongoing innovation and improvement in MEL methods. Furthermore, to further improve the adaptability of MEL methods, we introduce a modality-augmented training strategy with which we fine-tune the $CLIP (ViT-B/32)$~\cite{clip} model. This strategy, by expanding the expressiveness of modal features, augments the training process. Following experimentation and analysis, the \textit{CLIP\_N\_D} model obtained after training demonstrates significant performance improvements in ACC, with an average increase of 9.3\% to 25\%. This illustrates the considerable potential of the modal enhancement strategy in handling multi-modal data and emphasizes the research value of the $M^3EL$ dataset.


To summarize, the main contributions of this work are as follows:
\begin{itemize}
\item[1.] We present a large-scale manually labelled high-quality dataset, $M^3EL$, which covers a diverse range of topics and supports various multi-modal tasks.
\item[2.] We propose a modality-augmented training strategy. Based on this strategy, we use the $M^3EL$ dataset as a corpus to train a $CLIP (ViT-B/32)$ model, resulting in $CLIP\_N\_D$, which further improves the model's performance in multi-modal entity linking.
\item[3.] Experimental results indicate that our proposed large-scale, multi-task, multi-topic, multi-modal dataset serves as a high-quality pre-training corpus. While effectively enhancing the model's generalization performance, our dataset still presents a challenging benchmark.
\end{itemize}


==> raw_file/analysis.tex <==
\section{Analysis and Discussion}

\subsection{Effect of Tool Adaptation.}
\label{sec:Effect of Tool Adaptation.}
In Table \ref{tab: Tool Adaption}, we compare different semantic understanding prompts. It is evident that Prompt 5-0 achieved the best results. Due to the use of Wikidata to search for LLM outputs (referred to as query) in Prompt 3-0 and 4-0, while 5-0 searches for mentions, this proves that excessively long search fields can diminish the quality of candidates. The precision of Prompt 4-0 significantly surpassed that of Prompt 3-0. Due to the fact that Prompt 4-0 integrates in-context learning examples derived from Wikidata, while Prompt 3-0 relies on the original dataset for its learning examples. This discrepancy suggests that Wikidata furnishes more contemporary and precise entity information. Prompt 3-1 (4-1) significantly outperforms Prompt 3-0 (4-0). When searching Wikidata for a query with no results, Prompt 3-1 (4-1) uses a mention as a substitute for the query for a second search. In all Prompts, the precision in Men is higher than Doc. These results further proves the effectiveness of entity-level searches on Wikidata, searching mentions within Wikidata can yield better candidates.

\begin{table}[!t]
\caption{\textbf{Effect of Tool Adaptation.} X tokens represent the length used to segment document, Sen represents linking all mentions in a sentence at once; Men means linking only one mention in a sentence.}
\label{tab: Tool Adaption}
\centering
\setlength{\tabcolsep}{4mm}{\begin{tabular}{ccccc}
\toprule
    \multirow{2}{*}{\textbf{Prompts}}& \multicolumn{2}{c}{\textbf{64 tokens}} & \multicolumn{2}{c}{\textbf{128 tokens}} \\
          \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    &Sen & Men & Sen & Men  \\ \hline
    Prompt 3-0  &0.14  & 0.16  & 0.15  & 0.18 \\
    Prompt 3-1  &0.27  & 0.30  & 0.31  & 0.38 \\
    Prompt 4-0  &0.31  & 0.33  & 0.30  & 0.32 \\
    Prompt 4-1  &0.56  & 0.57  & 0.56  & 0.58 \\
    Prompt 5-0  &0.65  & 0.66  & 0.67  & 0.68 \\
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[!t]
\caption{\textbf{Effect of Candidate Filtering.} BLEU and BERTScore are similarity metrics.}
\label{tab: Candidate Filtering}
\centering
\setlength{\tabcolsep}{4mm}{\begin{tabular}{ccccc}
\toprule
    \multirow{3}{*}{\textbf{Similarity}} & \multicolumn{4}{c}{\textbf{Prompt 3-1}} \\ 
        \cline{2-5} 
        & \multicolumn{2}{c}{64 tokens} & \multicolumn{2}{c}{128 tokens} \\ 
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & Sen           & Men           & Sen            & Men           \\ \hline
        BLEU       & 0.54  & 0.55  & 0.53  & 0.58 \\
        BERTScore  & 0.60  & 0.61  & 0.62  & 0.64 \\ 
    \midrule[0.8pt]
    \midrule[0.8pt]     
    \multirow{3}{*}{\textbf{Similarity}} & \multicolumn{4}{c}{\textbf{Prompt 4-1}} \\
        \cline{2-5} 
        & \multicolumn{2}{c}{64 tokens} & \multicolumn{2}{c}{128 tokens} \\ 
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & Sen           & Men           & Sen            & Men           \\ \hline
        BLEU        & 0.60  & 0.62  & 0.62  & 0.65  \\
        BERTScore   & 0.64  & 0.66  & 0.67  & 0.69  \\
\bottomrule
\end{tabular}}
\end{table}


\subsection{Effect of Candidate Filtering.}
% To access the candidate quality of each Prompt, we use BLEU \cite{bleu} and BERTScore \cite{sentence-bert} to filter candidates. 
In Table \ref{tab: Candidate Filtering}, we employ BLEU \cite{bleu} and BERTScore \cite{sentence-bert} to calculate $sim(query, description)$ for filtering candidates, where $query$ is the output of the semantic understanding prompt and $description$ is candidate’s attribute in wikidata.

Primarily, the candidates set filtered by similarity significantly improves the precision of linking. Specifically, in Prompt 3-1, precision saw a twofold increase, and in Prompt 4-1, precision was on average boosted by 5.5\%. Second, the effect of using BERTScore is significantly better than BLEU. In Prompt 3-1, precision was on average increased by 6.8\%, and in Prompt 4-1, there was an average improvement of 4.3\%. Finally, the results show that Men is more accurate than Doc. 

These results show that using a similarity filtering mechanism improves linking accuracy by selecting candidates. Furthermore, the candidates are the search results of wikidata, this method avoids extra computational costs and the need to store and navigate the target knowledge graph, achieving low-resource objectives.




\begin{table}[!t]
\centering
\caption{\textbf{Effect of Multiple Choice.} Mul. Cho. and Str. Mat. are short for Multiple Choice and String Match.}
\label{ablation for AIDA}
\setlength{\tabcolsep}{5mm}{\begin{tabular}{ccc}
\toprule
    \textbf{Datasets} &\textbf{Str. Mat.} &\textbf{Mul. Cho.} \\ \hline
    AIDA-B      &0.67   &0.85  \\
    WNED-Wiki   &0.44   &0.73  \\
    WNED-Cweb   &0.42   &0.73  \\
    Wiki-Wiki   &0.60   &0.76  \\
\bottomrule
\end{tabular}}

\end{table}

\subsection{Effect of Multiple Choice. }
As illustrated in Table \ref{ablation for AIDA}, the use of multiple choice prompt for linking outperforms the traditional string matching approach. In the WNED-Cweb dataset, there is a maximal precision increase of 31\%. Due to the dataset containing a large volume of single-character mentions (e.g., m), which challenge traditional models' filtering capabilities. However, LLM improve precision by using their semantic understanding abilities with multiple-choice prompt. In the wikiwiki dataset, the minimum precision increase is 16\%, as the mentions are mainly tangible daily objects (e.g., water) with few semantically ambiguous ones. This indicates that LLM contains extensive knowledge and excel in semantic understanding beyond traditional matching models. Using GPT-3.5 and multiple choice prompt, entity linking can be efficiently accomplished without requiring substantial computational resources for training and storing specialized models.


==> raw_file/approach.tex <==
\section{Approach}
In this section, we introduce LLMA-EL, an effective framework designed for online and unsupervised EL, with the aim of improving the performance of conventional unsupervised EL methods. The overview of our framework is shown in Figure \ref{fig:overview}.

\begin{figure*}[]
    \centering
    \includegraphics[width=1\textwidth]{figures/cikm_model.pdf}
    \caption{\textbf{The overview of our LLMA-EL.} The Semantic Understanding module consists of two main components: utilizing the Wikidata tool and the Semantic Understanding Agent for mention comprehension. The Multi-Round Candidate Adaptation module comprises an adaptive iteration strategy for candidates and the Multi-choice Agent.}
    \label{fig:overview}
\end{figure*}

\subsection{Overview}
The key steps in EL include candidate generation and re-ranking. Traditional models typically employ small-scale pretrained models to generate candidates from specific static knowledge graphs, but these models struggle to achieve high accuracy and coverage due to limited semantic understanding. Moreover, most existing studies opt for a cold handling strategy when the correct answer is missing from the candidates, reducing the robustness of the model in practical applications. 

Our framework improves the quality of candidates by utilizing tool calls and innovative semantic understanding cues. In addition, an adaptive iterative strategy for candidates improves their accuracy and the use of multiple choice cues in task transitions increases the accuracy of links.
In Section ~\ref{sec:Tool Adaptation}, we analyze how to optimize the use of Wikidata. In Section ~\ref{sec:Candidates Generation}, we discuss how to process Wikidata search results to obtain more accurate candidates. In Section ~\ref{sec:Candidates Adaptive Iteration}, we describe our strategy for updating candidates through iteration when the correct answer is absent. Finally, in Section ~\ref{sec:Multiple Choice}, we transform the re-ranking task into a multiple-choice format to enhance the efficiency of EL. By integrating Wikidata search with the iterative and selection processes of LLMs, and utilizing advanced models like ChatGPT, we significantly enhance the performance of EL.

\subsection{Tool Adaptation}
\label{sec:Tool Adaptation}
\textbf{Decompose Task Granularity by split(mention). } As the foundational model, LLM has strong natural language processing capabilities. However, its limitations on input context length can restrict application scope and efficiency. As discussed in \textit{Effect of Tool Adaptation} in Section ~\ref{sec:Further Analysis}, this text length limitation may result in truncated outputs, thereby compromising the completeness and accuracy of EL.


% Use Input in the format of Algorithm
\renewcommand{\algorithmicrequire}{\textbf{Input:}} 
% Use Output in the format of Algorithm  
\renewcommand{\algorithmicensure}{\textbf{Output:}}  

\begin{algorithm}
\caption{\textbf{: Sentence-level EL}}
\vspace{-0.11cm} 
\begin{algorithmic}[1]
\label{alg:Sentence-level-EL}
\REQUIRE{ 
A document $\mathcal{D}$; a mention set $\mathcal{M}_{\textit{D}}$ and its mentions $m$, $m \in \mathcal{M}_{\textit{D}}$; a LLM model $\mathcal{L}$; \par

\hspace{1.28em} a template $\mathcal{T}$ for EL prompting.}

\ENSURE {A candidate set $Cans$ for mention $m(s)$.

\STATE {$//$ Divide $\mathcal{D}$ based on $\mathcal{M}_{\textit{D}}$}}

    \FOR{$m \in \mathcal{M}_{\textit{D}}$}
        \STATE $s(m) \gets split(D)$
    \ENDFOR

    \STATE {$//$ Get a sentence set $\mathcal{S}_{\textit{D}}$}
    
    \STATE $\mathcal{S}_{\textit{D}} \gets$ a sentence set for $\mathcal{D}$; \par
    \hspace{2.5em}$s \in \mathcal{S}_{\textit{D}}$ \par
    \hspace{2.5em} the sentence's mention $ m(s) $

    \STATE {$//$ Traversing $\mathcal{S}_{\textit{D}}$ for EL}    
    
    \FOR{$s \in \mathcal{S}_{\textit{D}}$}
        \STATE $\mathcal{P} \gets \mathcal{T}(s,m(s))$;
        \STATE $Cans(s) \gets \mathcal{L(\mathcal{P})}$
    \ENDFOR

\end{algorithmic}
\end{algorithm}
% \vspace{-0.3cm}

For this issue, we were inspired by the least-to-most prompting method~\cite{least-to-most}, which enhances EL by decomposing document-level task into sentence-level tasks. Given a document $\mathcal{D}$, we use the target mentions as the basis for task segmentation, dividing the entire document into a sentence set $\mathcal{S}_{\textit{D}}$, where each sentence $s_i$ contains a single mention $m$. The EL process follows a repetitive linking paradigm outlined in Algorithm ~\ref{alg:Sentence-level-EL}.




\noindent \textbf{Adapt Tool by Semantic Understanding Prompt. } 
By decomposing tasks, the context of each mention is the sentence to which it belongs. When employing online Wikidata for searching mentions within a sentence, since Wikidata functions as an entity-level search engine, obtaining search results becomes unfeasible. If online Wikidata is exclusively utilized for mention searches, inaccuracies arise due to semantic ambiguities within the mentions, thus hindering the retrieval of precise search outcomes.

In order to better adapt to the search tool, online Wikidata, we have constructed a semantic understanding prompt, which comprises the sentence of mention and comprehension logic. LLM acts as a semantic understanding agent to comprehend information related to mention according to the requirements of the prompt, achieving nuanced understanding and semantic disambiguation when necessary. 
% For instance, in the sentence ‘\textit{Soccer-late goals give JAPAN win over SYRIA.}’ the mention ‘\textit{JAPAN}’ carries ambiguity, referring to the '\textit{Japan national football team}' rather than the ‘\textit{country}’ itself. By comprehending the semantic understanding prompt and acquiring understanding: ‘\textit{The target mention 'JAPAN' refers to a soccer team or national team from Japan, which emerged victorious in a soccer match against Syria.}’, as shown in Figure \ref{fig:overview} ($\mathrm{II}$).


\subsection{Candidates Generation}
\label{sec:Candidates Generation}

\textbf{Candidate Search based on Tool Invocation.} We leverage the online version of Wikidata as our target knowledge graph. However, online Wikidata functions as an entity-level search engine. For instance, utilizing Wikidata to search for ‘\textit{Soccer-late goals give JAPAN win over SYRIA.}’ or ‘\textit{The target mention 'JAPAN' refers to a soccer team ...}’ fails to retrieve the entity: \textit{Japan national football team (Q170566)}. Based on this attribute, we employed Wikidata to search for mention  (e.g., JAPAN) from the sentence and obtain all candidates, as shown in Figure \ref{fig:overview} ($\mathrm{I}$). Here, we limit the number of candidates to no more than 200.

\noindent \textbf{Candidate Filtering used similarity metrics.}
Through the candidate search process, we obtained 200 candidates related to the target mention '\textit{JAPAN}'. The information associated with these candidates includes their name, Q\_id, and description, among other attributes. We selected the top-5 retrieval candidates to form the set $Sea\_can$, as illustrated by yellow dashed box in Figure ~\ref{fig:overview}. Due to the semantic ambiguity inherent in the mention '\textit{JAPAN}', as illustrated in Figure \ref{fig:overview} ($\mathrm{III}$), it can be observed that the returned candidates encompass unrelated entities such as the Japanese nation and Japanese history, among others.

In Section ~\ref{sec:Tool Adaptation} we elucidate the tool adaptation, a step through which semantic summaries of mentions can be obtained. To further refine the scope of candidates and reduce irrelevant candidates, we employ a filtering mechanism based on the similarity between the understanding of mentions and the descriptions of candidates. We utilize BLEU ~\cite{bleu} and BERTScore ~\cite{sentence-bert} as metrics to calculate the similarity of the understanding-description pair, selecting the top-5 candidates with the highest similarity scores, forming the set $Sim\_can$, as illustrated by blue dashed box in Figure \ref{fig:overview}.

Thus, the final candidate set $Cans$ can be represented as follows:
\begin{equation}
    Cans = \{ Sea\_can \cap Sim\_can \}.
    \label{eq:1}
\end{equation}

We defer the detailed experiments regarding the specific selection and combination of candidates to Experiments section.

\subsection{Candidates Adaptive Iteration}
\label{sec:Candidates Adaptive Iteration}
% \textbf{Candidates Updating by Adaptive Iterative Strategy.} 
After acquiring the candidate set $Cans$, the LLM acts as a judgment agent, assessing whether the candidate set contains the correct entity corresponding to the mention in the document. If the candidate set includes the correct entity, the process moves to the multiple-choice stage. If not, the current candidate set is fed back into the semantic comprehension agent, integrating the candidates into the semantic prompts. The LLM then revises its understanding of the mention based on this feedback and iteratively rebuilds the candidate set based on the updated understanding, continuing until the large model confirms the presence of the correct entity in the set, at which point the iteration ceases.

\subsection{Multiple Choice}
\label{sec:Multiple Choice}
% \textbf{Entity Linking by Multiple Choice Prompt.}
The LLM refers to deep neural network model trained on extensive datasets, which exhibit enhanced NLP capabilities and superior generative performance compared with traditional machine learning models. Consequently, we transform the string matching task using ML models into a multiple-choice task with LLMs.

The multiple choice prompt was constructed, as shown in purple box in Figure ~\ref{fig:overview} ($\mathrm{V}$). The prompt consists of four components, where [SENTENCE] refers to the sentence where the mention is located, [TARGET MENTION] represents the mention to be linked, [OPTIONS] represents all the choices within the candidate set $Cans$ for the multiple-choice question, and [SELECT BEST OPTION] indicates the requirement for the multiple-choice question. Based on this multiple choice prompt, employ LLM ChatGPT for selection.



==> raw_file/dataset-raw.tex <==
\section{Data Setups for $\boldsymbol{M^3EL}$}

% \begin{figure*}[!h]
%     \centering
%     \includegraphics[width=1\textwidth]{Figures/pipline.pdf}
%     \caption{The overview of $M^3EL$ data pipline.}
%     \label{fig:overview}
% \end{figure*}

The framework of the data construction pipeline of $M^3EL$ is illustrated in Figure 1. In the following, we detail the construction of $M^3EL$.

% It mainly comprises 4 steps.
% \begin{itemize}
% \item [1)] ~\textbf{Raw Data Acquisition:} The first step is to collect extensive raw data from Kaggle~\footnote{\url{https://www.kaggle.com/}} and filter it to build the data foundation of $M^3EL$ which are JSON, CSV and Pickle files with mention information, covering 5 topics.
% \item [2)] ~\textbf{Mention Curation:} In this step, we extract mentions and its context from the raw data, and use the URL attribute to navigate to Wikidata~\footnote{\url{https://www.wikidata.org/wiki/Wikidata:Main_Page}} for retrieving QID, description and other relevant information of mentions.
% \item [3)] ~\textbf{Candidate Construction:} Using Wikidata to search for mentions, the first 100candidates are obtained as the initial candidates, and the final candidates is constructed by rigorously filtering the candidates based on the completeness of the textual and visual information.
% \item [4)] ~\textbf{Image Crawling:} A code framework for image crawling is constructed based on Wikidata, Wikipedia~\footnote{\url{https://www.wikipedia.org/}}, Wikimedia~\footnote{\url{https://commons.wikimedia.org/wiki/Main_Page}} and BDpedia~\footnote{\url{https://www.dbpedia.org/}}. The CLIP model was then employed to filter the scraped images, selecting those most relevant to the mention.
% \end{itemize}

% In the following, we detail the construction of $M^3EL$.

\subsection{Data Collection}
\noindent \textbf{Raw data Acquisition. \quad}To construct the foundational dataset for $M^3EL$, we collected raw data from Kaggle~\footnote{\url{https://www.kaggle.com/}} that includes URL information related to DBpedia~\footnote{\url{https://www.dbpedia.org/}}, Wikipedia~\footnote{\url{https://www.wikipedia.org/}}, or Wikidata~\footnote{\url{https://www.wikidata.org/wiki/Wikidata:Main_Page}}. These data files are diverse in format, including JSON, CSV, Pickle, and more. Since DBpedia, Wikipedia and Wikidata pages can interlink, where Wikidata's QID attributes can be used as entity labels, these datasets are well-suited as raw data sources for research in multi-modal entity linking. In addition, these Kaggle datasets are derived from real-world data science scenarios and cover a wide range of topics, reflecting the complexity and diversity of data in the real world. Specifically, we utilized \textit{the Wikipedia Movie Plots}~\footnote{\url{https://www.kaggle.com/datasets/jrobischon/wikipedia-movie-plots?select=wiki_movie_plots_deduped.csv}} dataset as the raw data for the movies topic, the \textit{Wiki-Wiki}~\footnote{\url{https://drive.google.com/file/d/1Oebe1sbbixX7FWHX813diCdqReh1IyWH/view}} dataset for common knowledge topic, the \textit{People Wikipedia Data}~\footnote{\url{https://www.kaggle.com/datasets/sameersmahajan/people-wikipedia-data}} for person topic, the \textit{Books Datasets}~\footnote{\url{https://www.kaggle.com/datasets/saurabhbagchi/books-dataset}} for book topic, and the \textit{AIDA-CoNLL-Test}~\footnote{\url{https://www.mpi-inf.mpg.de/departments/databases-and-information-systems/research/ambiverse-nlu/aida/downloads}} for the sports topic.

\noindent \textbf{Data Filter and clean. \quad}For the raw dataset, we performed the following data cleaning steps: 1) Removed non-English expressions and single-character mentions. 2) Deleted mentions without associated images or whose images could not be downloaded. Following these pre-processing steps, we finally obtained a total of 82K mentions, each comprising a text-image pair, which serves as the base dataset for $M^3EL$.


\subsection{Data Curation}
\noindent \textbf{Mention Curation. \quad} 
Due to the varying formats of raw data across different topics, we describe in detail the process of obtaining relevant mentions for each topic separately.

For the raw data on the movie topic, we utilized the "Title" attribute from the \textit{wiki\_movie\_plots\_deduped.csv} file to extract movie titles as mentions. The "Plot" attribute was employed to provide contextual information related to these mentions. Additionally, we accessed the mention-related Wikipedia pages through the URLs provided in the "Wiki Page" attribute. From these Wikipedia pages, we further navigated to the corresponding Wikidata pages to obtain fundamental information, including the QID and descriptions.

For the raw data on commons topic, we utilized the instances provided by the "Target" attribute in the \textit{wikihow.csv} file as mentions, and paragraphs provided by the "Text" attribute as contextual information for mentions. By constructing a mention semantic understanding prompt, we input it into the large language model GPT-4 to obtain semantic information related to the mentions. Subsequently, each mention was searched in Wikidata, and the Wikidata entry that best matches the mention is filtered based on the semantic information obtained from GPT-4, and relevant information such as QID and description is obtained.

For the raw data on person topic, we utilized the \textit{people\_wiki.csv} file, specifically the "name" attribute, as the reference for mentions, and the "text" attribute, which provides the context for these mentions. The associated DBpedia pages were accessed via the "URL" attribute. Subsequently, we navigated to the corresponding Wikidata pages to obtain foundational information, including the QID and descriptions.

For the raw data on book topics, we utilized the "Book-Title" attribute of the \textit{books.csv} file as a mention for searching the corresponding Wikidata pages to retrieve basic information, including the QID and description. To ensure the accuracy of the search results, we cross-validated them using the Book-Author, Year of Publication, and Publisher information provided in the file. Mentions that could not be found on the Wikidata page were subsequently removed.

For the raw data on sport topic, the \textit{AIDA\_B\_dict\_} \textit{raw.pickle} file provides mentions, contextual information, and associated QID information in Wikidata in the form of a dictionary. We directly utilized the textual information from the raw data without any processing.

\noindent \textbf{Candidate Construction. \quad} 
In most entity linking tasks, Wikidata is used as the target Knowledge Graph, linking mentions to their corresponding entities. However, due to the large scale of Wikidata, which contains approximately 95 million entries, matching every mention by traversing all entities would consume substantial computational resources and time. Therefore, to enhance the quality and usability of the dataset, we employ an optimization strategy: for each mention, a refined subset is filtered from Wikidata to serve as the candidate set. This set contains both possible and incorrect corresponding candidates, which truly reflects the challenges of the multi-modal entity linking task.

The specific steps are as follows: 1) We search for the mention surface on the Wikidata page and retrieve the top 100 relevant search results. For each search result, we access its Wikidata detail page and systematically extract the key information, including the entity's QID, entity name, and description, among other textual data. 2) We enter the stage of obtaining candidate entity images, and when the number of candidates satisfying complete textual and visual information reaches a predetermined threshold of $k$, the candidate set construction is completed. This process ensures the completeness of the information and the high quality of the dataset, which provides a solid foundation for the subsequent data analysis and model training.

\noindent \textbf{Image Crawling. \quad} 
After obtaining the mention-related textual information of different topics, in order to obtain the image information corresponding to the mentions, we developed a comprehensive image crawling frameworks based on Wikidata, Wikipedia and Wikimedia~\footnote{\url{https://commons.wikimedia.org/wiki/Main_Page}} pages. Furthermore, we utilized a pre-trained \textit{CLIP} (\textit{ViT}-\textit{B}-\textit{32}) model to effectively filter the most relevant images by leveraging the joint representation of visual and textual information. Especially for the book topic, we directly use the URLs of book covers provided in the raw data to obtain relevant images. For invalid URLs, we implemented a supplementary crawler that automatically searches for and retrieves relevant images using book titles as keywords on Goodreads~\footnote{\url{https://www.goodreads.com}} and Amazon ~\footnote{\url{https://www.amazon.com}}. These steps ensure that we are able to obtain the appropriate image information for each mention, enriching the multi-modal characteristics of the dataset.

\subsection{Data Analysis}
\noindent \textbf{Size and Difficulty Measure. \quad}
The statistics of $M^3EL$ dataset in detail are shown in Table~\ref{table:Data_Analysis}. This dataset was constructed from 66,342 articles and contains a total of 79K entities, covering 316K images. Each entity is mapped to a specific entity in Wikidata. Notably, many entities appear multiple times in different sentences of the articles, ensuring that the entities can be fully learned. In addition, Figure~\ref{figure: Statistics_of_type}(a) reports the distribution of entity topics. Unlike existing MEL datasets, which are typically constructed for specific scenarios or tasks, $M^3EL$ covers 5 distinct topics and involves 9 types of multi-modal linking tasks. These tasks include $T_m$-$T_e$, $T_m$-$I_e$, $T_m$-($I$+$T)_e$, $I_m$-$T_e$, $I_m$-$I_e$, $I_m$-($I$+$T)_e$, ($I$+$T)_m$-$T_e$, ($I$+$T)_m$-$I_e$, ($I$+$T)_m$-($I$+$T)_e$, making it a more comprehensive and diverse dataset.

Firstly, we compare the surface form similarity between mentions and ground-truth entities. It is observed that 41.3\% of the mentions differ from the surface forms of the ground-truth entities. This significant discrepancy in surface forms presents a challenge for multi-modal entity linking tasks. Secondly, we report the candidates for each mention in Figure~\ref{figure: Statistics_of_type}(b). Intuitively, the larger the candidate set of entities involved in a mention, the more ambiguous the semantics of the mention is, which in turn leads to a decrease in the accuracy of EL or MEL. Specifically, based on the co-occurrence statistics of (m, e) from Wikidata, we generate a candidate set $C$ for each mention $m$. As shown in Figure~\ref{figure: Statistics_of_type}(b), we observe the following: 1) 55.8\% of mentions have three candidates, with 55.8\% of these mentions having the correct entity ranked first in the candidate set, and 29.4\% having the correct entity ranked elsewhere within the candidate set. 2) 14.8\% of mentions have candidate sets that do not include the correct entity. This indicates that the candidate set reflects the real-world scenarios of entity linking to a certain extent.

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\toprule
\textbf{Topic} & \textbf{Documents} & \textbf{Mention} & \textbf{Candidate} & \textbf{Image} & \textbf{Tasks} \\ \midrule
Movie & 32131 & 32800 & 98400 & 131200 & \multirow{7}{*}{9} \\ \cmidrule{1-5}
Common & 1699 & 11826 & 35478 & 47304 &  \\ \cmidrule{1-5}
Person & 26873 & 24278 & 72834 & 97112 &  \\ \cmidrule{1-5}
Book & 5408 & 7276 & 21828 & 29104 &  \\ \cmidrule{1-5}
Sport & 231 & 3445 & 10335 & 13780 &  \\ \midrule
ALL & 66342 & 79625 & 238875 & 318500 & 9 \\ \bottomrule
\end{tabular}%
}
\caption{Statistics of $M^3EL$. Documents represent the raw textual contexts of mentions, Tasks refers to 9 different multi-modal tasks.}
\label{table:Data_Analysis}
\end{table}

\noindent \textbf{Diversity of multi-modal tasks. \quad}
Compared to existing datasets, $M^3EL$ offers a more comprehensive range of multi-modal tasks. Traditional multi-modal entity linking datasets, such as Snap~\cite{moon-etal-2018-multimodal-named}, Twitter~\cite{adjali-etal-2020-building}, and Weibo~\cite{zhang2021attention}, are designed for specific tasks. Although datasets like WIKIPerson~\cite{sun2022visual} and WIKIDiverse~\cite{wang2022wikidiverse} introduce various forms of multi-modal entity linking tasks, including $I_m-T_e$, $I_m-I_e$, and $(I+T)_m-I_e$, they ignored other potential linking tasks. In contrast, $M^3EL$ significantly expands the scope of tasks, covering 9 distinct types, abbreviations: $T-T$, $T-I$, $T-IT$, $I-T$, $I-I$, $I-IT$, $IT-T$, $IT-I$, $IT-IT$. This task diversity greatly enhances MEL's ability to generalise across a wide range of multi-modal related tasks, enabling it to better accommodate the diverse needs of users in the real world.


\noindent \textbf{Coverage of topic types. \quad}
As illustrated in Table~\ref{table:existing_datasets}, most existing training datasets predominantly focus on a limited range of topic types, such as people and news. WIKIDiverse~\cite{wang2022wikidiverse} advances the state-of-the-art by developing a scraping framework to extract multi-modal information from Wikinews, thereby expanding multi-modal task types to include $T_m-T_e$,$I_m-I_e$,$I_m-T_e$,$(I+T)_m-I_e$ tasks. However, our $M^3EL$ dataset further diversifies these tasks by covering 9 different multi-modal entity linking tasks, encompassing all possible combinations of image and text modalities. Such comprehensive coverage makes M3EL more flexible in dealing with multi-modal entity linking tasks and improves its applicability in various application scenarios.

\begin{figure}[t]
    \centering
    \subfigure[\scriptsize{Entity topic distribution.}]{\includegraphics[width=0.19\textwidth]{Figures/type_distribution.pdf}}
    \hspace{0.1in}
    \subfigure[\tiny{Different type candiates distribution.}]{\includegraphics[width=0.25\textwidth]{Figures/candidates_distribution.pdf}}
    \caption{More statistics of $M^3EL$. (a) Entity topic type distribution. (b) Distribution of correct entity positions within the candidates.}
    \label{figure: Statistics_of_type}
\end{figure}

==> raw_file/exp_bak.tex <==
\section{Experiments}
\subsection{Datasets}

\begin{table*}
\begin{center}
\caption{\textbf{Datasets and their statistics.} The categories 'easy', 'hard', 'difficult', and 'none' each represent the different candidates for a mention: 'easy' means the correct answer is the first candidate; 'hard' means the correct answer is included but not first; 'difficult' means the correct answer is absent from the candidates; 'none' means no candidates are available. Additionally, 'max\_mention' refers to the maximum number of mentions in a single document.}
\label{tab:dataset}
\setlength{\tabcolsep}{0.6mm}{\begin{tabular}{cccccccc}
\toprule
    \multirow{2}{*}{\textbf{Datasets}}& \multicolumn{5}{c}{\textbf{Details of the mention}} & \multicolumn{2}{c}{\textbf{Details of the document}} \\
          \cmidrule(lr){2-6} \cmidrule(lr){7-8}
    &easy & hard & difficult & none & overall & max\_mention & overall \\ \midrule[1pt]
    AIDA-B &2534 (57\%) &1110 (25\%) &621 (15\%) &148 (3\%) &4413 &96 &231 \\
    WNED-WIKI &2731 (41\%) &1475 (22\%) &1722 (26\%) &766 (11\%)&6694 &46 &318 \\
    WNED-CWEB &4667 (42\%) &3056 (28\%) &2653 (24\%) &664 (6\%)&11040 &37 &320\\
    Wiki-Wiki &2727 (24\%) &8560 (76\%) &0 (-\%) &0 (-\%)&11287 &3 &7097 \\
\bottomrule
\end{tabular}}
\end{center}
\end{table*}



To better measure the performance of our framework, we used the same English dataset as the baseline for our experiments. The statistics of these datasets are shown in Table ~\ref{tab:dataset}.

\textbullet\ \hspace{0.2em}The \textbf{AIDA-CoNLL}\footnote{\url{https://www.mpi-inf.mpg.de/departments/databases-and-information-systems/research/ambiverse-nlu/aida/downloads}} dataset \cite{AIDA} stands as one of the earliest high-quality manually annotated datasets within the entity linking literature. It is founded on the CoNLL 2003 shared task ~\cite{CoNLL-2003}. This dataset is segmented into training, validation, and testing partitions. Given the entirely unsupervised nature of our framework, we solely utilize the testing (CoNLL-Test) subset.

\textbullet\ \hspace{0.2em}The \textbf{WNED-Wiki}\footnote{\url{http://dx.doi.org/10.7939/DVN/10968}} and \textbf{WNED-Cweb(WNED-Clueweb)}\footnotemark[\value{footnote}] datasets are introduced benchmark datasets by ~\cite{WNED}, which were created by uniformly sampling mentions with different levels of prior scores from English Wikipedia (‘2013-06-06’ dump) and FACC1 \footnote{\url{http://lemurproject.org/clueweb12/}} respectively.

\textbullet\ \hspace{0.2em}The \textbf{Wiki-Wiki}\footnote{\url{https://drive.google.com/file/d/1Oebe1sbbixX7FWHX813diCdqReh1IyWH/view?usp=sharing}} dataset ~\cite{SumMC} consist mentions of common sense knowledge extraced from the WikiHow\footnote{\url{https://www.wikihow.com/Main-Page}} and their corresponding entity to Wikidata.


\subsection{Baselines}
We consider three kinds of models as baselines. First, as our task does not rely on annotated data, we chose the first EL model $\tau$MIL-ND \cite{MIL-ND} that is not based on annotated data. Second, given that our framework operates entirely without supervision, we compare it with Eigentheme \cite{Eigentheme}, the inaugural model in the domain of unsupervised entity linking (EL). Last, we employ ChatGPT, which is an EL approach harnessing the capabilities of LLM, and compare it to other LLM-based EL methods SumMC \cite{SumMC}. 

\textbullet\ \hspace{0.2em}\textbf{$\tau$MIL-ND}: The $\tau$MIL-ND, designed by \cite{MIL-ND}, represents one of the earliest EL models that does not require annotated datasets. It transforms the EL task into a binary multi-instance learning (MIL) task by employing a noise-based detection classifier with remote supervision

\textbullet\ \hspace{0.2em}\textbf{Eigentheme}: The Eigentheme, designed by \cite{Eigentheme}, stands out as the most mature solution in the realm of fully unsupervised EL tasks. By constructing the full embedding space for entities through graph embeddings, the model identifies the low-rank subspace using Singular Value Decomposition (SVD) and calculates candidate entities based on their proximity to the subspace.

\textbullet\ \hspace{0.2em}\textbf{SumMC}: The SumMC model, as designed by \cite{SumMC}, is a pioneering model that was the first to employ a LLM (GPT-3) to achieve a fully unsupervised EL task. Currently, it represents the state-of-the-art among fully unsupervised EL models.

%For further information on the baselines, please refer to Appendix ~\ref{sec:appendix B}.

\subsection{Implementation Details}
\textbf{Knowledge Graph. } In our framework, we primarily consider the Wikidata\footnote{\url{https://wikidata.org/}}. Wikidata is a knowledge graph complementing Wikipedia\footnote{\url{https://en.wikipedia.org/}} (providing rich encyclopedic information about world entities), which structures and organizes this encyclopedic knowledge in relational triples.

\noindent \textbf{Large Language Models. } In our task, due to the higher costs and limitations associated with the use of GPT-4, we employ the powerful LLM ChatGPT (GPT-3.5-turbo) by default in this paper, which is accessed by the OpenAI API\footnote{\url{https://platform.openai.com/}}. We prompt LLMs with instructions and in-context examples, requiring outputs in JSON format. The details of different prompts are shown in Appendix ~\ref{sec:appendix G}.

\noindent \textbf{Experimental Setups. } We use OpenAI API to call ChatGPT, where the temperature parameter is set to 0.75 (for consistency in fixed output formats) and the maximum token length for the input is set to 256. We use 32 shots in the semantic understanding prompt and 2 shots in the multiple choice prompt and the maximum number of iterations was limited to 5 for the candidates adaptive iteration. Wikidata is used as the source KG, and the number of search results is set to 200. In all experiments, we use the metric precision \texttt{@}1 to evaluate the effectiveness of EL.

\subsection{Main Results}

\begin{table*}[!t]\small
\caption{\textbf{Comparison with Baselines.} EL effectiveness assessed  through precision\texttt{@}1. 
Easy, Hard, and Diff (abbreviation for Difficult) serve as three question difficulty modes. Easy includes questions where the correct answer as the first option, Hard includes questions where the correct answer beyonds the first option, and Diff includes questions with both correct and incorrect answers. Mul. Cho. and Can. Fil. are short for Multiple Choice and Candadite Filtering. Bold and underline fonts denote the best and second best methods.}
\label{tab:baselines}
\centering
\begin{tabular}{ccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{MODELS}} & \multicolumn{3}{c}{\textbf{AIDA-B}} & \multicolumn{3}{c}{\textbf{WNED-Wiki}} & \multicolumn{3}{c}{\textbf{WNED-Cweb}} & \multicolumn{3}{c}{\textbf{Wiki-Wiki}} \\
                        & Easy    & Hard    & Diff   & Easy        & Hard        & Diff       & Easy         & Hard         & Diff        & Easy        & Hard        & Diff       \\ \hline
$\tau$MIL-ND  & 0.70    & 0.19    & 0.45   & -        & -        & 0.13    & -         & -         & 0.27     & -        & -        & 0.31    \\
Eigentheme  & \underline{0.86}    & 0.50    & 0.62   & 0.82     & 0.47     & 0.44    & 0.77      & 0.41      & 0.29     & 0.61     & 0.53     & 0.50    \\
SumMC       & 0.80    & 0.71    & 0.64   & 0.81     & 0.65     & 0.47    & 0.75      & 0.60      & 0.48     & 0.62     & \underline{0.80}     & \underline{0.76}    \\
ChatGPT     & 0.29    & 0.26    & 0.25   & 0.12     & 0.10     & 0.10    & 0.22      & 0.20      & 0.20     & 0.18     & 0.15     & 0.14    \\ \hline
w/o Can. Fil. & 0.40    & 0.35    & 0.33   & 0.26     & 0.22     & 0.21    & 0.33      & 0.27      & 0.28     & 0.26     & 0.25     & 0.23    \\
w/o Ada. Int.   & 0.81    & 0.70    & 0.65   & 0.81     & 0.68   &0.66    & 0.76      &0.63    &0.67   &0.64     &0.76   &0.70    \\
w/o Mul. cho.    & \underline{0.86}    & \underline{0.74}    & \underline{0.78}   & \underline{0.84}     & \underline{0.69}     & \underline{0.69}    & \underline{0.79}      &\underline{0.63}      & \underline{0.67}     & \underline{0.66}     & \underline{0.80}     & \underline{0.76}    \\


LLMA-EL        & \textbf{0.89}    & \textbf{0.76}    & \textbf{0.80}   & \textbf{0.87}     & \textbf{0.71}     & \textbf{0.72}    & \textbf{0.80}      & \textbf{0.65}      & \textbf{0.68}     & \textbf{0.69}     & \textbf{0.83}     & \textbf{0.77}    \\ \bottomrule
\end{tabular}
\end{table*}


\begin{figure*}
\includegraphics[width=\linewidth]{figures/compare_candidates.pdf} 
\caption{\textbf{Compare the quality of candidates for all datasets.} The definitions of easy, hard, and difficult align with those in Table \ref{tab:baselines}, where none indicates no candidates. The green line shows the distribution of candidates in the raw dataset, while the red line shows the changes in the distribution of candidates after LLMA-EL processing.}
\label{fig:Compare-can-dataset}
\end{figure*}


There are three question modes (Easy, Hard and Diificult) for entity linking (see Table \ref{tab:baselines} for details). We continue to employ the results of $\tau$MIL-ND and Eigentheme from \cite{Eigentheme}, utilizing publicly available datasets. The results of SumMC are collected from \cite{SumMC}. The specific results are presented in Table \ref{tab:baselines}.

\textbf{Comparison with Previous EL Models.} LLMA-EL achieves more competitive performance than other unsupervised EL models on four datasets. 

On the AIDA-B, WNED-Wiki, and WNED-Cweb datasets, we observed that Eigentheme demonstrates remarkable performance when dealing with Easy questions. This advantage stems from its ability to grasp the global context by leveraging the relationships between mentions, thereby highlighting the inherent information within the mention and enhancing its effectiveness in handling Easy questions. However, Eigentheme ignores the context within the document. In contrast, LLMA-EL constructs semantic understanding prompt and leverages the robust comprehension capabilities of the LLM. It comprehends mentions based on the entirety of document information, without requiring additional training of a semantic model. LLMA-EL implemented superior performance than Eigentheme on Easy question, with a 2\% improvement in precision at its best.

On the AIDA-B and Wiki-Wiki datasets, SumMC performs outstandingly when handling Hard questions. This benefits from SumMC's ability to leverage LLM to condense document information into concise sentences relevant to mentions, thereby enriching the contextual information around mentions and enhancing its capability to address Hard questions. Nevertheless, the SumMC model did not take into account the importance of semantic disambiguation. LLMA-EL outperforms SumMC's performance on Hard questions by incorporating in-context learning examples in its semantic understanding prompts. It concurrently achieves semantic disambiguation while summarizing mention information. In the best case, it improves 2\% precision.

In all datasets, the baseline assumes that Easy $\cup$ Hard equals Diff. Given the weak semantic understanding of pre-trained models based on similarity matching and the static nature of traditional knowledge graphs, which are incomplete and inaccurate, many multiple-choice questions lack correct options or have no options available. In contrast, LLMA-EL adopts a different strategy by categorizing questions with no correct options or no options as Diff issues and treating them uniformly. This system searches online Wikipedia data to obtain the latest and most accurate information, using the results as candidate options. Through an adaptive iterative strategy, the system optimizes the candidate set, significantly reducing the proportion of such issues and improving the accuracy of handling Diff problems.


\textbf{Comparison with ChatGPT. }  The ‘ChatGPT’ in Table \ref{tab:baselines} evaluates the ability of GPT-3.5 to independently perform EL task. Specifically, we first annotate the mention in document as $[mention]$, then input the annotated document to the model, and require the model to return all the corresponding entities of annotated mentions and their Q\_id in Wikidata at once. Experimental results indicate that the GPT-3.5 performs poorly in the task of linking all mentions in a document at once. Firstly, due to the limited input text length, a complete output cannot be guaranteed. Secondly, the model's knowledge is limited by temporal restrictions, preventing it from accessing the most current entities in Wikidata. This emphasizes the importance of task decomposition.

\textbf{Comparison of Different Operations of LLMA-EL} 'LLMA-EL w/o Can. Fil.' directly queries Wikidata for candidates, the experiments show that candidates matched without semantic understanding agent significantly decrease the precision of EL. This demonstrates the crucial role of LLMs' robust semantic capabilities in comprehending mentions in documents and filtering candidates, effectively mitigating the semantic limitations of smaller models.

'LLMA-EL w/o Ada. Int.' refers to executing the framework only once, without iterative judgment on the candidates filtered by semantic understanding agent. Experimental results indicate that further enhancement of candidate quality is achieved through an adaptive iteration strategy for candidates.

'LLMA-EL w/o Mul. Cho.' annotates mention in the document as $[mention](can 1)(can 2)...(can N)$, where the candidates are iteratively updated. The document is fed into the LLM, which outputs a selected candidate. Results show that constructing multiple-choice prompt better utilizes the linking capabilities of LLM.


\textbf{The Quality of Candidates.} In Figure \ref{fig:Compare-can-dataset}, by comparing the quantities of candidates across different categories, we observe a significant efficiency of LLMA-EL in boosting the quality of candidates. In the AIDA, WNED-WIKI, and WNED-CWEB datasets, the implementation of LLMA-EL has markedly improved the quality of candidates, substantially elevating the quantities of those classified as ‘easy’ and ‘hard’, whilst concurrently effecting a notable reduction in the instances of candidates deemed ‘difficult’ and ‘none’. For the Wiki-Wiki dataset, the performance is relatively average. This is because the Wiki-Wiki dataset is manually annotated by \cite{SumMC} and contains only ‘easy’ and ‘hard’ categories. Due to the inherent error rate in LLM's reading comprehension and the stringent search requirements of Wikidata, some mentions from ‘easy’ and ‘hard’ categories are erroneously classified as ‘difficult’. This underscores the significance of dynamic online knowledge graphs.




\subsection{Analysis and Discussion}

\textbf{Effect of Tool Adaptation.} In Table \ref{tab: Tool Adaption}, we compare different semantic understanding prompts. It is evident that Prompt 5-0 achieved the best results. Due to the use of Wikidata to search for LLM outputs (referred to as query) in Prompt 3-0 and 4-0, while 5-0 searches for mentions, this proves that excessively long search fields can diminish the quality of candidates. The precision of Prompt 4-0 significantly surpassed that of Prompt 3-0. Due to the fact that Prompt 4-0 integrates in-context learning examples derived from Wikidata, while Prompt 3-0 relies on the original dataset for its learning examples. This discrepancy suggests that Wikidata furnishes more contemporary and precise entity information. Prompt 3-1 (4-1) significantly outperforms Prompt 3-0 (4-0). When searching Wikidata for a query with no results, Prompt 3-1 (4-1) uses a mention as a substitute for the query for a second search. In all Prompts, the precision in Men is higher than Doc. These results further proves the effectiveness of entity-level searches on Wikidata, searching mentions within Wikidata can yield better candidates.

\begin{table}[!t]
\caption{\textbf{Effect of Tool Adaptation.} X tokens represent the length used to segment document, Sen represents linking all mentions in a sentence at once; Men means linking only one mention in a sentence.}
\label{tab: Tool Adaption}
\centering
\setlength{\tabcolsep}{4mm}{\begin{tabular}{ccccc}
\toprule
    \multirow{2}{*}{\textbf{Prompts}}& \multicolumn{2}{c}{\textbf{64 tokens}} & \multicolumn{2}{c}{\textbf{128 tokens}} \\
          \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    &Sen & Men & Sen & Men  \\ \hline
    Prompt 3-0  &0.14  & 0.16  & 0.15  & 0.18 \\
    Prompt 3-1  &0.27  & 0.30  & 0.31  & 0.38 \\
    Prompt 4-0  &0.31  & 0.33  & 0.30  & 0.32 \\
    Prompt 4-1  &0.56  & 0.57  & 0.56  & 0.58 \\
    Prompt 5-0  &0.65  & 0.66  & 0.67  & 0.68 \\
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[!t]
\caption{\textbf{Effect of Candidate Filtering.} BLEU and BERTScore are similarity metrics.}
\label{tab: Candidate Filtering}
\centering
\setlength{\tabcolsep}{4mm}{\begin{tabular}{ccccc}
\toprule
    \multirow{3}{*}{\textbf{Similarity}} & \multicolumn{4}{c}{\textbf{Prompt 3-1}} \\ 
        \cline{2-5} 
        & \multicolumn{2}{c}{64 tokens} & \multicolumn{2}{c}{128 tokens} \\ 
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & Sen           & Men           & Sen            & Men           \\ \hline
        BLEU       & 0.54  & 0.55  & 0.53  & 0.58 \\
        BERTScore  & 0.60  & 0.61  & 0.62  & 0.64 \\ 
    \midrule[0.8pt]
    \midrule[0.8pt]     
    \multirow{3}{*}{\textbf{Similarity}} & \multicolumn{4}{c}{\textbf{Prompt 4-1}} \\
        \cline{2-5} 
        & \multicolumn{2}{c}{64 tokens} & \multicolumn{2}{c}{128 tokens} \\ 
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & Sen           & Men           & Sen            & Men           \\ \hline
        BLEU        & 0.60  & 0.62  & 0.62  & 0.65  \\
        BERTScore   & 0.64  & 0.66  & 0.67  & 0.69  \\
\bottomrule
\end{tabular}}
\end{table}


\textbf{Effect of Candidate Filtering.} In Table \ref{tab: Candidate Filtering}, we employ BLEU \cite{bleu} and BERTScore \cite{sentence-bert} to calculate $sim(query, description)$ for filtering candidates, where $query$ is the output of the semantic understanding agent and $description$ is candidate’s attribute in wikidata.

Primarily, the candidates set filtered by similarity significantly improves the precision of linking. Specifically, in Prompt 3-1, precision saw a twofold increase, and in Prompt 4-1, precision was on average boosted by 5.5\%. Second, the effect of using BERTScore is significantly better than BLEU. In Prompt 3-1, precision was on average increased by 6.8\%, and in Prompt 4-1, there was an average improvement of 4.3\%. Finally, the results show that Men is more accurate than Doc. 

The experimental results demonstrate that candidates filtered based on the similarity between queries and descriptions, extracted using semantic understanding agents, show significantly improved quality. This approach effectively addresses the weaknesses of smaller pre-trained language models in terms of candidate accuracy and coverage comprehensiveness due to weak semantic comprehension.




\begin{table}[!t]
\centering
\caption{\textbf{Effect of Multiple Choice.} Mul. Cho. and Str. Mat. are short for Multiple Choice and String Match.}
\label{ablation for AIDA}
\setlength{\tabcolsep}{5mm}{\begin{tabular}{ccc}
\toprule
    \textbf{Datasets} &\textbf{Str. Mat.} &\textbf{Mul. Cho.} \\ \hline
    AIDA-B      &0.67   &0.85  \\
    WNED-Wiki   &0.44   &0.73  \\
    WNED-Cweb   &0.42   &0.73  \\
    Wiki-Wiki   &0.60   &0.76  \\
\bottomrule
\end{tabular}}

\end{table}

\textbf{Effect of Multiple Choice.} As illustrated in Table \ref{ablation for AIDA}, the use of multiple choice prompt for linking outperforms the traditional string matching approach. In the WNED-Cweb dataset, there is a maximal precision increase of 31\%. Due to the dataset containing a large volume of single-character mentions (e.g., m), which challenge traditional models' filtering capabilities. However, LLM improve precision by using their semantic understanding abilities with multiple-choice prompt. In the wikiwiki dataset, the minimum precision increase is 16\%, as the mentions are mainly tangible daily objects (e.g., water) with few semantically ambiguous ones. This indicates that LLM contains extensive knowledge and excel in semantic understanding beyond traditional matching models. Using GPT-3.5 and multiple choice prompt, entity linking can be efficiently accomplished without requiring substantial computational resources for training and storing specialized models.


==> raw_file/exp_copy.tex <==
\section{Experiments}
\subsection{Primarily}
\noindent \textbf{Task Formulation \quad}
Let \( E \) represent the set of entities in the Knowledge Graph (\textit{KG}), typically comprising millions of entities. Let \( C \) denote the candidate set in the \textit{KG} for each mention \( m \), where \( C \subseteq E \). Each mention \( m \) or entity \( e \in C \) is associated with its corresponding visual context \( V_m \), \( V_e \), and textual context \( T_m \), \( T_e \). Here, \( T_m \) and \( T_e \) denote the textual context surrounding \( m \) and \( e \), respectively. \( V_m \) refers to the images related to \( m \), while \( V_e \) refers to the images associated with \( e \) in the \textit{KG}. Therefore, the multi-modal task of identifying the corresponding entity for mention \( m \) can be defined as follows: 

\begin{table}[!h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c}
\toprule
$\bm{M_m}$ & $\bm{M_e}$ & \textbf{Multi-modal Tasks} \\ \midrule
$T_m$ & $T_e$ & $T_m - T_e \ \vert\  T_m - I_e  \ \vert\  T_m - (I+T)_e$ \\ \midrule
$I_m$ & $I_e$ & $I_m - T_e  \ \vert\   I_m - I_e  \ \vert\  I_m - (I+T)_e$ \\ \midrule
$(I+T)_m$ & $(I+T)_e$ & $(I+T)_m - T_e \ \vert\  (I+T)_m - I_e  \ \vert\  (I+T)_m - (I+T)_e$ \\ \bottomrule
\end{tabular}%
}
\caption{Introduction to different modal information and modal tasks. $T_m$ ($T_e$) denotes the textual information of the mention (entity), while $I_m$ ($I_e$) represents the visual information of the mention. $(I+T)_{m(e)}$ refers to the combined textual and visual information of the mention (entity).}
\label{table:different_modal_combine}
\end{table}


\begin{equation}
    S(M_m,M_e) = \mathop{\arg\max} \limits_{e_i \in C}\Psi(En(M_m), En(M_e)),
    \label{eq:1}
\end{equation}
where $M_m$ and $M_e$ represents the modal information of the target mention $m$ and the candidate entity $e$, respectively, as detailed in Table 3. The function \( f \) denotes the similarity score between the $m$ and the $e$.

\noindent \textbf{\textit{CLIP} Definition \quad}
The Contrastive Language–Image Pre-training (\textit{CLIP}) method has demonstrated significant effectiveness in training visual models using language supervision. In each training step, a large batch of $N$ pairs of images and texts \(\{x_I, x_T\}\) is randomly sampled from the training dataset. Subsequently, data augmentation is applied to the images to simulate various real-world visual variations. The augmented images and their corresponding texts are then processed by dedicated encoders and normalization functions \(f_I\) and \(f_T\) to extract image and text features. These features are utilized to compute the InfoNCE loss, a type of contrastive loss that distinguishes between matched (positive) and mismatched (negative) image-text pairs. The training loss is represented by the following equation:

\begin{equation}
    L = \sum_{i=1}^N \log \frac{exp(sim(f_I(aug_I(x_I^i)), f_T(x_T^i))/ \tau)}{\sum_{j=1}^N exp(sim(f_I(aug_I(x_I^j)), f_T(x_T^j))/ \tau)},
    \label{eq:2}
\end{equation}

where $(x_I^i, x_T^i)$ represents the $i$-th image-text pair, and $aug_I()$ denotes the image augmentation function. The $sim(-, -)$ function measures similarity using the dot product, while the temperature parameter $\tau$ is a learnable variable used to scale the logits.

\noindent \textbf{Enhanced Strategy \quad}
In Equation~\ref{eq:2}, while the standard \textit{CLIP} loss applies augmentation to images to enhance the model's adaptability and robustness to visual variations, the textual input remains constant throughout the training process. This approach ignores the potential diversity and ambiguity inherent in textual data. To address this issue, we propose a strategy to augment the textual data with entity description information, denoted as $aug_T$, where \(x_T\) is replaced by $aug_T(x_T)$ as the input to \(f_T\). By applying text augmentation, more detailed and precise textual information is input into the model, enhancing its ability to handle semantic ambiguities and ultimately improving its performance on multi-modal tasks.


\subsection{Experimental Setups}

\noindent \textbf{Datasets \quad}
For multi-modal entity linking tasks, it is necessary to link mentions from different modalities to specific entities in a KG. However, most existing multi-modal entity linking datasets are relatively small in scale and contain limited types of cross-modal tasks, such as $I_m-I_e$ and $T_m-T_e$. To address these limitations, we constructed a new dataset named $M^3EL$, which consists 79,625 instances, all of which have been manually annotated. In total, we collected 318,500 images accompanied by textual captions. The $M^3EL$ dataset has been divided into training, validation, and test sets in the ratio of 8:1:1.

To further verify the quality of the constructed dataset, we also investigated other existing multi-modal datasets:

\begin{itemize}
    \item {\textbf{DiffusionDB}~\cite{wangDiffusionDBLargescalePrompt2022}} is the first large-scale text-to-image cue dataset. It contains 14 million images generated by Stable Diffusion using real user-specified cues and hyperparameters. We chose a subset of this dataset "2m\_random\_1k", which contains 1000 image-text pairs, primarily aimed at the task of $I_m-T_e$.
    \item {\textbf{WIKIPerson}~\cite{sun2022visual}} is a high-quality visual person linking dataset designed for Visual Named Entity Linking tasks. Unlike existing entity linking datasets, each mention is represented solely by an image containing a PERSON entity, corresponding to a unique entity in Wikipedia. We selected a test set containing 6,142 images, along with their labels (the corresponding Wikidata QIDs) and descriptions. This dataset primarily facilitates tasks such as $I_m-T_e$, $I_m-I_e$, and $I_m-(I+T)_e$.
    \item {\textbf{WIKIDiverse}~\cite{wang2022wikidiverse}} is a high-quality, manually annotated MEL dataset consisting of diverse contextual topics and entity types derived from Wikinews. The dataset includes 8 image-caption pairs and utilizes Wikipedia as the corresponding KG. We have selected a test set comprising 1,570 image-caption pairs, primarily designed to implement $T_m-T_e$, $I_m-I_e$, $(I+T)_m-I_e$ and $(I+T)_m-(I+T)_e$ tasks.
\end{itemize}


\noindent \textbf{Baselines \quad}
Given the diverse range of modality tasks encompassed by our proposed multi-modal dataset, the number of comparable models is notably limited. In order to establish a valid benchmark for evaluation, we report on the performance of several state-of-the-art methods for entity linking and visual entity recognition, including \textit{ALIGN}~\cite{align}, \textit{BLIP-2}~\cite{blip2}, \textit{CLIP}~\cite{clip}, \textit{FLAVA}~\cite{flava}, \textit{OWL-ViT}~\cite{OWL-ViT}, and \textit{SigLIP}~\cite{siglip}. Additionally, we present our own optimized approach, \textit{CLIP\_N\_D}.


\noindent \textbf{Implementation Details \quad}
We utilized the CLIP model pre-trained on ImageNet as our foundational model. Specifically, we employed the ViT-B/32 architecture, which comprises both text and image encoders, each with a hidden state dimension of 768 and 12 multi-head attention mechanisms. We trained on an A100 GPU with 40GB of memory with 35 epochs and a batch of 256. The AdamW optimizer was applied with an initial learning rate of 1e-5, betas=(0.9, 0.98), eps=1e-6, and weight\_decay=0.001.

% \subsection{Evaluation Metric}
\noindent \textbf{Evaluation Metric \quad}
The primary metric we evaluate is the accuracy (ACC) of linking entities to KG entities. Accuracy is defined by the following formula:

\begin{equation}
    ACC = \frac{\sum_{i=1}^{N_{correct}} M_m-M_e}
    {\sum_{i=1}^{N} M_m-M_e},
    \label{eq:4}
\end{equation}

where $N_{correct}$ represent the number of correctly linked entity mentions, $N$ represent the total number of mentions, $M_m-M_e$ denotes different modalities of mention-entity linking task. 

\subsection{Experimental Results}

\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\toprule
\textbf{} & \textbf{Diffusion} & \textbf{WIKIPerson} & \textbf{WIKIDiverse} & \textbf{M3EL} \\ \midrule
\textbf{ALIGN} & 0.468 & \underline{0.826} & 0.707 & 0.683 \\
\textbf{BLIP-2} & 0.552 & 0.652 & 0.677 & \underline{0.746} \\
\textbf{CLIP} & 0.517 & \underline{0.873} & 0.762 & 0.758 \\
\textbf{FLAVA} & 0.582 & 0.529 & \underline{0.718} & 0.655 \\
\textbf{OWL-ViT} & 0.421 & 0.348 & \underline{0.609} & 0.494 \\
\textbf{SigLIP} & 0.539 & \underline{0.771} & 0.743 & 0.724 \\
\textbf{CLIP\_N\_D} & \textbf{0.724} & \underline{\textbf{0.916}} & \textbf{0.796} & \textbf{0.897} \\ \bottomrule
\end{tabular}%
}
\caption{Experimental results of the baseline models on each dataset. the best-performing model on each dataset is highlighted in bold, while the best performance of each model across different datasets is indicated with an underline.}
\label{table: Experimental_results}
\end{table}


\begin{table*}[!h]
\small
\centering
\begin{tabular}{ccccccccc}
\toprule
 & $S\_1$ & $S$ & $M\_S_1$ & $M\_S$ & $S_1\_M$ & $S\_M$ & $S_1\_M\_D$ & $S\_M\_D$ \\ \midrule
ALIGN & 0.674 & 0.675 & 0.683 & 0.683 & 0.680 & 0.681 & 0.701 & 0.697 \\
BLIP-2 & 0.738 & 0.739 & 0.745 & 0.746 & 0.743 & 0.744 & 0.759 & 0.753 \\
CLIP & 0.742 & 0.748 & 0.754 & 0.758 & 0.749 & 0.753 & 0.771 & 0.763 \\
FLAVA & 0.654 & 0.649 & 0.661 & 0.655 & 0.659 & 0.653 & 0.681 & 0.699 \\
OWL-ViT & 0.487 & 0.487 & 0.495 & 0.494 & 0.489 & 0.488 & 0.490 & 0.492 \\
SigLIP & 0.711 & 0.714 & 0.722 & 0.724 & 0.715 & 0.717 & 0.736 & 0.726 \\
CLIP\_N\_D & \textbf{0.885} & \textbf{0.882} & \textbf{0.899} & \textbf{0.897} &\textbf{ 0.890} &\textbf{ 0.888} & \textbf{0.902} & \textbf{0.898} \\ \bottomrule
\end{tabular}%
\caption{Experimental results of the baseline model on various $M^3EL$ versions.The $M^3EL$ dataset comes in various versions, each made up of composite text and images. $M$ indicates the mention's surface, $S$ its full context, $S_1$ a single sentence with the mention, and $D$ the mention's description. Formats include $M-S$ (mention: sentence), $S-M$ (sentence mention), and $S-M-D$ (sentence mention: description).}
\label{table:various_M3EL_versions}
\end{table*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{Figures/ablation.pdf}
    \caption{Ablation study to analyze modality absence of mention’s different textual information. W/o T\_name or T\_description stands for CLIP\_N\_D trained without the corresponding inputs.}
    \label{fig:ablation}
\end{figure}


\noindent \textbf{Main Results \quad}
In Table~\ref{table: Experimental_results}, we report the accuracy of the model in detail. Based on the experimental results, we observe that our trained multi-modal approach, \textit{CLIP\_N\_D}, outperforms all baseline methods that rely solely on the raw modal information, especially in the dataset WIKIPerson, where the accuracy is improved by 4.3\% to 56.8\%. This significant performance boost is primarily attributed to the augmented feature strategy implemented during the training process. Secondly, except for the \textit{BLIP-2} model, other models did not achieve the highest link accuracy on the $M^3EL$. Compared to the best-performing model, these models exhibited an average accuracy deficit of 7.6\%. Lastly, the model performed the worst on the Diffusion dataset, due to the ambiguous mentions in the textual information paired with images, making linking more hard. Models performed most consistently in the WIKIDiverse, as the surface of mentions in the text-image pairs were more explicit. Most models performed best in the dataset WIKIPerson, due to the availability of bounding boxes within images where the mentions were located, allowing the models to access more specific and accurate image features. Overall, the $M^3EL$ dataset combines the strengths of various datasets by providing clear mention and diverse text-image features, which helps enhance the generalization ability of multi-modal models.


\noindent \textbf{Further Analysis \quad}
In Table~\ref{table:various_M3EL_versions}, we provide a comprehensive analysis of multi-modal task performance on the $M^3EL$. The experimental results are shown: Firstly, our CLIP-finetune achieves significant performance improvements over the baseline model on different versions of the multi-modal dataset. Specifically, on the M-S form, \textit{CLIP\_N\_D} demonstrated a 13.9\% increase in accuracy compared to the baseline, with an average improvement of 7\% across other datasets. Notably, \textit{CLIP\_N\_D} and \textit{CLIP} share identical parameters and computational costs during training. Secondly, when auxiliary text information (e.g., entity names and descriptions) is added to the multi-modal task, the linking accuracy of the baseline model increases significantly, by an average of 1.2\%. This suggests that the level of detail and clarity of the auxiliary text plays a key role in enhancing the model ability. Thirdly, all models consistently performed better when utilizing the $S_1\_M\_D$ format for multimodal tasks compared to the $S\_M\_D$ format. This is mainly due to the $S_1\_M\_D$ format's ability to convey more precise information about the entities. In contrast, the $S\_M\_D$ format may truncate key entity and description information due to text length limitations, thereby negatively impacting model performance. Additionally, while most models perform better on multimodal tasks that contain richer textual information ($S$format), for models focusing on visual modality such as FLAVA and OWL-ViT, more textual information may introduce noise and degrade link performance.


\noindent \textbf{Ablation Analysis \quad}
We conducted an ablation study, and the experimental results are presented in Figure~\ref{fig:ablation}. It is evident that the model achieves optimal performance when it utilizes both mentions' name and description information as multi-modal context. In contrast, models trained using only a single source of information (e.g., only name or description) performed poorly. In addition, an interesting phenomenon was observed in the experiments: when the model used only sentences $S_1$ involving mentions as context, the performance was better than using complete sentences $S$. This suggests that models trained with text augmentation strategies have better comprehension in capturing semantic information related to mentions, whereas the use of longer texts may introduce noise, which reduces model performance.

\subsection{Further Analysis}
\label{sec:Further Analysis}
\textbf{Effect of Tool Adaptation.} In Table \ref{table: Experimental_results}, we compare different semantic understanding prompts. It is evident that Prompt 5-0 achieved the best results. Due to the use of Wikidata to search for LLM outputs (referred to as query) in Prompt 3-0 and 4-0, while 5-0 searches for mentions, this proves that excessively long search fields can diminish the quality of candidates. The precision of Prompt 4-0 significantly surpassed that of Prompt 3-0. Due to the fact that Prompt 4-0 integrates in-context learning examples derived from Wikidata, while Prompt 3-0 relies on the original dataset for its learning examples. This discrepancy suggests that Wikidata furnishes more contemporary and precise entity information. Prompt 3-1 (4-1) significantly outperforms Prompt 3-0 (4-0). When searching Wikidata for a query with no results, Prompt 3-1 (4-1) uses a mention as a substitute for the query for a second search. In all Prompts, the precision in Men is higher than Doc. These results further proves the effectiveness of entity-level searches on Wikidata, searching mentions within Wikidata can yield better candidates.

\begin{table}[!t]
\caption{\textbf{Effect of Tool Adaptation.} X tokens represent the length used to segment document, Sen represents linking all mentions in a sentence at once; Men means linking only one mention in a sentence.}
\label{tab: Tool Adaption}
\centering
\small
\setlength{\tabcolsep}{4mm}{\begin{tabular}{ccccc}
\toprule
    \multirow{2}{*}{\textbf{Prompts}}& \multicolumn{2}{c}{\textbf{64 tokens}} & \multicolumn{2}{c}{\textbf{128 tokens}} \\
          \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    &Sen & Men & Sen & Men  \\ \hline
    Prompt 3-0  &0.14  & 0.16  & 0.15  & 0.18 \\
    Prompt 3-1  &0.27  & 0.30  & 0.31  & 0.38 \\
    Prompt 4-0  &0.31  & 0.33  & 0.30  & 0.32 \\
    Prompt 4-1  &0.56  & 0.57  & 0.56  & 0.58 \\
    Prompt 5-0  &0.65  & 0.66  & 0.67  & 0.68 \\
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[!t]
\caption{\textbf{Effect of Candidate Filtering.} BLEU and BERTScore are similarity metrics.}
\label{tab: Candidate Filtering}
\small
\centering
\setlength{\tabcolsep}{4mm}{\begin{tabular}{ccccc}
\toprule
    \multirow{3}{*}{\textbf{Similarity}} & \multicolumn{4}{c}{\textbf{Prompt 3-1}} \\ 
        \cline{2-5} 
        & \multicolumn{2}{c}{64 tokens} & \multicolumn{2}{c}{128 tokens} \\ 
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & Sen           & Men           & Sen            & Men           \\ \hline
        BLEU       & 0.54  & 0.55  & 0.53  & 0.58 \\
        BERTScore  & 0.60  & 0.61  & 0.62  & 0.64 \\ 
    \midrule[0.8pt]
    \midrule[0.8pt]     
    \multirow{3}{*}{\textbf{Similarity}} & \multicolumn{4}{c}{\textbf{Prompt 4-1}} \\
        \cline{2-5} 
        & \multicolumn{2}{c}{64 tokens} & \multicolumn{2}{c}{128 tokens} \\ 
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & Sen           & Men           & Sen            & Men           \\ \hline
        BLEU        & 0.60  & 0.62  & 0.62  & 0.65  \\
        BERTScore   & 0.64  & 0.66  & 0.67  & 0.69  \\
\bottomrule
\end{tabular}}
\end{table}


\textbf{Effect of Candidate Filtering.} In Table \ref{tab: Candidate Filtering}, we employ BLEU ~\cite{bleu} and BERTScore ~\cite{sentence-bert} to calculate $sim(query, description)$ for filtering candidates, where $query$ is the output of the semantic understanding agent and $description$ is candidate’s attribute in wikidata.

Primarily, the candidates set filtered by similarity significantly improves the precision of linking. Specifically, in Prompt 3-1, precision saw a twofold increase, and in Prompt 4-1, precision was on average boosted by 5.5\%. Second, the effect of using BERTScore is significantly better than BLEU. In Prompt 3-1, precision was on average increased by 6.8\%, and in Prompt 4-1, there was an average improvement of 4.3\%. Finally, the results show that Men is more accurate than Doc. 

The experimental results demonstrate that candidates filtered based on the similarity between queries and descriptions, extracted using semantic understanding agents, show significantly improved quality. This approach effectively addresses the weaknesses of smaller pre-trained language models in terms of candidate accuracy and coverage comprehensiveness due to weak semantic comprehension.




\begin{table}[!t]
\centering
\caption{\textbf{Effect of Multiple Choice.} Mul. Cho. and Str. Mat. are short for Multiple Choice and String Match.}
\label{ablation for AIDA}
\small
\setlength{\tabcolsep}{5mm}{\begin{tabular}{ccc}
\toprule
    \textbf{Datasets} &\textbf{Str. Mat.} &\textbf{Mul. Cho.} \\ \hline
    AIDA-B      &0.67   &0.85  \\
    WNED-Wiki   &0.44   &0.73  \\
    WNED-Cweb   &0.42   &0.73  \\
    Wiki-Wiki   &0.60   &0.76  \\
\bottomrule
\end{tabular}}

\end{table}

\textbf{Effect of Multiple Choice.} As illustrated in Table \ref{ablation for AIDA}, the use of multiple choice prompt for linking outperforms the traditional string matching approach. In the WNED-Cweb dataset, there is a maximal precision increase of 31\%. Due to the dataset containing a large volume of single-character mentions (e.g., m), which challenge traditional models' filtering capabilities. However, LLM improve precision by using their semantic understanding abilities with multiple-choice prompt. In the wikiwiki dataset, the minimum precision increase is 16\%, as the mentions are mainly tangible daily objects (e.g., water) with few semantically ambiguous ones. This indicates that LLM contains extensive knowledge and excel in semantic understanding beyond traditional matching models. Using ChatGPT as a multi-choice agent, based on multi-choice prompt, can more specifically and efficiently leverage the capabilities of LLMs in entity linking tasks.

\textbf{The Quality of Candidates for Candidate Filtering.} In our research, both Prompt 3-1 and Prompt 3-0 employ Wikidata to search for the outputs (queries) of semantic understanding prompts. When the initial search yields no results, Prompt 3-1 utilizes a mention as a substitute to conduct a second search. The processing logic for Prompt 4-1 and Prompt 4-0 follows the same methodology. Upon comparison, we found that Prompt 3-1 and Prompt 4-1 respectively outperform Prompt 3-0 and Prompt 4-0 in terms of performance. Thus we compare the quality of candidates between Prompt 3-1 and Prompt 4-1 across various document segmentation by token (64 or 128) in Figure \ref{fig:p1+p2}. Each subfigure presents three distinct scenarios of candidate filtering:

\begin{itemize}
    \item {\textbf{w.o. Can. Fil. : }}Without using Candidate Filtering. Utilizing the term ‘understanding’ returned by semantic understanding agent as the query, call the dynamic online wikidata to directly search for the query, and obtain the results as the candidates.
    \item {\textbf{BLEU: }}Based on the results of tool invocation and semantic understanding prompt, use BLEU to calculate the similarity of understanding-description pair for filtering candidates.
    \item {\textbf{BERTScore: }}Similar to the step of BLEU.
\end{itemize}


\begin{figure}[htbp]
  \begin{subfigure}{0.9\linewidth}
	\centering
	\begin{subfigure}{\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/3-64-128.pdf}
        \caption{The candidates of Prompt 3-1}
		\label{logical}
	\end{subfigure}
 
	\begin{subfigure}{1\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/4-64-128.pdf}
        \caption{The candidates of Prompt 4-1}
		\label{physical}
	\end{subfigure}
	
  \end{subfigure}
  
\caption{\textbf{Quality Demonstration Graph of Candidates for Candidate Filtering.}} 
\label{fig:p1+p2}
\end{figure}


\begin{table*}[]
\caption{\textbf{The different examples in semantic understanding prompts.}}
\small
\label{tab:prompt3vs4}
\begin{tabular}{c|l}
\toprule
\textbf{Prompts} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Examples of semantic understanding prompt\\ (sentence, description)\end{tabular}}}                                                  \\ \midrule[1pt]
Prompt 3-1       & \begin{tabular}[c]{@{}l@{}}'Soccer-late goals give JAPAN win over SYRIA...',\\  'Japan national football team: national association football team.'\end{tabular}                          \\ \hline
Prompt 4-1       & \begin{tabular}[c]{@{}l@{}}'Soccer-late goals give JAPAN win over SYRIA...', \\ "Japan national football team: men's national association football team representing Japan."\end{tabular} \\
\bottomrule
\end{tabular}
\end{table*}

It becomes evident that candidates filtered with BLEU and BERT-Score are much better in quality than those without filtering (denoted as w.o. Can. Fil.). Specifically, the number of candidates containing the correct answer (both easy and hard) increases, while the number of candidates without the correct answer (difficult) and those yielding no search results (none) decreases. 
% This is primarily due to the search feature of Wikidata. Wikidata, being a knowledge graph rich in structured knowledge, is adept at searching for entities and their attribute information. Notably, when the target mention aligns closely with the entity name, Wikidata's precision in returning results is higher. However, using queries actually increases the complexity of the Wikidata search. For instance, when searching for ‘\textit{JAPAN}’, Wikidata returns ‘\textit{Japan (Q17)}’ representing the country, and when searching for ‘\textit{The target mention 'JAPAN' refers to a soccer team or national team from Japan, which emerged victorious in a soccer match against Syria.}’, Wikidata returns ‘\textit{There were no results matching the query}’. Therefore, direct search for query from semantic understanding prompt struggle to effectively complete semantic disambiguation and entity linking at once.
Comparing the quality of candidate by BLEU and BERTScore in Prompt 3-1 and Prompt 4-1, it becomes evident that BERTScore outperforms BLEU. This is because BLEU calculates the word repetition of query and description without considering semantic information. However, ChatGPT is a generative model that conveys understanding in the form of natural language, and the pre-trained BERT model can effectively capture semantic information of understanding and descriptions. 
In addition, under the same conditions, the candidate quality of Prompt 4-1 is better than that of Prompt 3-1. This variation is attributed to the different examples of in-context learning provided in each Prompt, which leads to distinct understandings of the mention and influences the similarity scores calculated by BLEU and BERTScore, ultimately affecting candidate quality. 

Table \ref{tab:prompt3vs4} presents an example constituted by a \textbf{tuple (sentence, description)}, where the \textbf{sentence}, indicating the context of the mention, remains consistent between Prompt 3-1 and Prompt 4-1. However, the \textbf{description} in Prompt 3-1 is derived from the original dataset's explanation of the mention, while the \textbf{description} in Prompt 4-1 comes from Wikidata's description of the mention. Given that descriptions from Wikidata are more current and accurate, the original dataset's explanations may contain errors due to their temporal limitations. Consequently, the candidate quality in Prompt 4-1 is superior to that in Prompt 3-1, further underscoring the necessity of utilizing online dynamic Wikidata as a replacement for the original static dataset (knowledge graph).



% \textbf{Different $Sea\_can$ \& $Sim\_can$.} In Table ~\ref{tab: Different combinations of cans}, we present different combinations of $Sea\_can$ and $Sim\_can$ used to construct the candidate sets $Cans$.

% \begin{itemize}
%     \item $Sea\_can$ refers to candidates that are constructed from the top-5 results obtained through searching mention on Wikidata.
%     \item $Sim\_can$ refers to candidates that are constructed from the top-5 results obtained through BERTScore(query, description).
%     \item $Sea\_can + Sim\_can$ refers to the candidates from $Sim\_can$ are appended to those in $Sea\_can$.
%     \item $Sim\_can + Sea\_can$ refers to the candidates from $Sea\_can$ are appended to those in $Sim\_can$.
% \end{itemize}

\textbf{Different $Sea\_can$ \& $Sim\_can$.} Table ~\ref{tab: Different combinations of cans} presents different combinations of $Sea\_can$ and $Sim\_can$ for constructing candidate sets $Cans$. $Sea\_can$ includes top-5 results from Wikidata search, while $Sim\_can$ includes top-5 results from BERTScore(query, description). Combining $Sea\_can$ and $Sim\_can$ (appending one to the other) improves precision, with $Sea\_can$ generally outperforming $Sim\_can$ due to Wikidata's robust search capabilities. Experiments showed that $Sea\_can + Sim\_can$ (Wikidata results first) yielded higher precision than $Sim\_can + Sea\_can$, as LLMs have a stronger memory for earlier-encountered information, enhancing multi-choice quality and entity linking precision.
% In Table ~\ref{tab: Different combinations of cans}, we present different combinations of $Sea\_can$ and $Sim\_can$ used to construct the candidate sets $Cans$. $Sea\_can$ refers to candidates that are constructed from the top-5 results obtained through searching mention on Wikidata. $Sim\_can$ refers to candidates that are constructed from the top-5 results obtained through BERTScore(query, description). $Sea\_can + Sim\_can$ refers to the candidates from $Sim\_can$ that are appended to those in $Sea\_can$, whereas $Sim\_can + Sea\_can$ refers to the candidates from $Sea\_can$ that are appended to those in $Sim\_can$.

% The precision of $Sea\_can$ surpasses that of $Sim\_can$. This superiority is attributable to Wikidata's robust search and matching capabilities, which yield higher quality results for mention searches. Additionally, when employing the BERTScore model, the model exhibits varying preferences for different vocabularies. Relying solely on the obtained candidates can inadvertently lower the correct candidate's rank among the candidates. Based on these observations, we conducted experiments involving the combination of two subsets of candidates.

% The precision of $Sea\_can + Sim\_can$ surpasses that of $Sim\_can + Sea\_can$, primarily due to the search results from Wikidata appearing in the upper half of the candidate list. The LLMs exhibit a deeper memory for information encountered earlier, which in turn enhances the quality of multi-choice, thereby increasing the precision of entity linking.


\begin{table}[]
\caption{\textbf{Different combinations of $Sea\_can$ and $Sim\_can$  to construct the $Cans$ in AIDA-B dataset.}}
\label{tab: Different combinations of cans}
\centering
\small
\setlength{\tabcolsep}{4mm}{\begin{tabular}{ccccc}
\toprule
    \multirow{2}{*}{\textbf{Combines}}& \multicolumn{2}{c}{\textbf{64 tokens}} & \multicolumn{2}{c}{\textbf{128 tokens}} \\
          \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    &Sen & Men & Sen & Men  \\ \hline
    $Sea\_can$               &0.65  & 0.66  & 0.67  & 0.68 \\
    $Sim\_can$               &0.47  & 0.49  & 0.51  & 0.54 \\ \hdashline
    $Sim\_can$ + $Sea\_can$  &0.56  & 0.59  & 0.61  & 0.64 \\
    $Sea\_can$ + $Sim\_can$  &0.69  & 0.71  & 0.70  & 0.78 \\
\bottomrule
\end{tabular}}
\end{table}



\begin{table}[]
\caption{\textbf{Effect of the different question of multiple choice prompt.} The can\_X indicates the number of candidates is X.}
\label{tab: different questions}
\centering
\small
\setlength{\tabcolsep}{3mm}{\begin{tabular}{cccc}
\toprule
    \textbf{Questions} &\textbf{Can\_5} &\textbf{Can\_10} &\textbf{Can\_20} \\ \hline
    sentence  &0.711   &0.774  &0.752  \\
    summary   &0.713   &0.774  &0.760\\
    understanding   &0.718   &0.783   &0.764\\
\bottomrule
\end{tabular}}
\end{table}


\begin{table}[htbp]
\caption{\textbf{The analysis of static offline knowledge graph lacks time-sensitive.} The "-X\%" denotes the random removal of X\% of data from the raw dataset.}
\label{tab:ablation for MC}
\centering
\small
\begin{tabular}{ccccc}
\toprule
    \textbf{Mentions} &\textbf{AIDA} &\textbf{WNED-Wiki} & \textbf{WNED-Cweb} & \textbf{Wiki-Wiki}  \\ \midrule[1pt]
    -70\%  &0.18  &0.14  &0.18  &0.27   \\
    -50\%  &0.35  &0.23  &0.26  &0.41   \\
    -30\%  &0.45  &0.30  &0.34  &0.52   \\ 
    -10\%  &0.56  &0.35  &0.36  &0.64   \\ \midrule[0.5pt] 
    all    &0.64  &0.47  &0.48  &0.76   \\
\bottomrule
\end{tabular}
\end{table}


\textbf{Different question of multiple choice.} In Table ~\ref{tab: different questions}, "sentence" denotes the sentence with the mention, "summary" comes from SumMC, and "understanding" is from LLMA-EL.

The results indicate that when employing the three terms as the question of multiple choice prompts for entity linking, the precision achieved by each prompt does not differ much. Notably, the precision of the understanding is marginally higher, attributable to the detailed steps incorporated within the semantic understanding prompt. These steps effectively exploit the LLM comprehension capability.

The number of candidates affects multiple-choice  results, with 10 candidates giving the best results. Having too few candidates (can\_5) means the correct option might not be covered. In contrast, having too many (can\_20) makes the text too long and complicates the selection process for LLMs due to their varied memory for differently sequenced information.

    
\textbf{Incompleteness of static knowledge graph}. In Table ~\ref{tab:ablation for MC}, we initiate an analysis of the impact of static offline knowledge graphs on the performance of the baseline SumMC. Specifically, we conducted experiments in which we randomly removed 10\%, 30\%, 50\%, and 70\% of mentions from the original dataset, simulating a scenario in which static offline knowledge graphs lack updates for mentions in the real world. 

The experimental results reveal that when a substantial number of unknown target mentions are present, the effectiveness of SumMC experiences a significant decline. For example, in the case of the Wiki-Wiki dataset, the removal of 70\% of target mentions results in a reduction of precision from 76\% to 27\%. Consequently, the invocation of tools, specifically the substitution of a static offline knowledge graph with a dynamic online KG, becomes highly necessary and meaningful.


==> raw_file/keywords.tex <==
\keywords{Entity linking, Knowledge graph, Large language model}
\keywords{Entity linking, Knowledge graph, Large language model}

==> sec/8-checklist.tex <==
\section{Reproducibility Checklist}
Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

This paper:

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA)
    
     \textbf{NA}
    
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no)

     \textbf{Yes}

    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no)

     \textbf{Yes}
    
\end{itemize}






Does this paper make theoretical contributions? (yes/no) If yes, please complete the list below.

 \textbf{Yes}

\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)

     \textbf{Yes}
    
    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
    
     \textbf{Yes}
    
    \item Proofs of all novel claims are included. (yes/partial/no)
    
     \textbf{Yes}
    
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
    
     \textbf{Yes}
    
    \item Appropriate citations to theoretical tools used are given. (yes/partial/no)
    
     \textbf{Yes}
    
    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
    
     \textbf{Yes}
    
    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
    
     \textbf{Yes}
    
\end{itemize}



Does this paper rely on one or more datasets? (yes/no) If yes, please complete the list below.

 \textbf{Yes}

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA)
    
     \textbf{Yes}
    
    \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)
    
     \textbf{NA}
    
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)
    
     \textbf{Yes}
    
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)
    
     \textbf{Yes}
    
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)
    
     \textbf{Yes}
    
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)
    
     \textbf{NA}
    
\end{itemize}


Does this paper include computational experiments? (yes/no) If yes, please complete the list below.

 \textbf{Yes}

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (yes/partial/no).
    
     \textbf{Yes}
    
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)
    
     \textbf{Yes}
    
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)
    
     \textbf{Yes}
    
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no)
    
     \textbf{Yes}
    
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)
    
     \textbf{NA}
    
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)
    
     \textbf{Yes}
    
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)
    
     \textbf{Yes}
    
    \item This paper states the number of algorithm runs used to compute each reported result. (yes/no)
    
     \textbf{Yes}
    
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)
    
     \textbf{Yes}
    
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)
    
     \textbf{Yes}
    
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)
    
     \textbf{Yes}
    
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. 
    (yes/partial/no/NA)
    
     \textbf{Yes}
    
\end{itemize}

